Why and How to Avoid the Flipped Quaternion Multiplication

Over the last decades quaternions have become a crucial and very successful tool for attitude representation in robotics and aerospace. However, there is a major problem that is continuously causing trouble in practice when it comes to exchanging formulas or implementations: there are two quaternion multiplications in common use, Hamilton's original multiplication and its flipped version, which is often associated with NASA's Jet Propulsion Laboratory. We believe that this particular issue is completely avoidable and only exists today due to a lack of understanding. This paper explains the underlying problem for the popular passive world to body usage of rotation quaternions, and derives an alternative solution compatible with Hamilton's multiplication. Furthermore, it argues for entirely discontinuing the flipped multiplication. Additionally, it provides recipes for efficiently detecting relevant conventions and migrating formulas or algorithms between them.

==> src/makefile <==
NAME=quatMult
MAINTEX=$(NAME).tex
STRIPPED=$(NAME)-source.tex

SOURCES=$(MAINTEX) *.tex *.bib makefile

FIGURES=rotation_conventions.pdf

$(NAME).pdf: $(SOURCES)
	pdflatex $<
	bibtex $(NAME)
	pdflatex $<
	pdflatex $<


used-figs.lst: $(SOURCES) 
	pdflatex $(MAINTEX) |grep '<figs/.*pdf' | sed 's/^.*\(figs\/.*\)\.pdf.*$$/\1/' > $@

$(STRIPPED): $(MAINTEX)
	sed '/^%/d' $< > $@
	
$(NAME)-source.bbl: $(NAME).bbl
	cp $< $@

FILES_FOR_ZIP=$(STRIPPED) $(NAME)-source.bbl *.bst *.cls notation-math-definitions.tex $(FIGURES) src/*

$(NAME).zip: $(FILES_FOR_ZIP)
	rm -f $@
	zip $(NAME).zip $(FILES_FOR_ZIP)

figs/%.eps:figs/%.pdf
	pdftops -eps $^ $@

.PHONY: test

test: $(NAME).zip
	rm -rf tmp/test
	mkdir tmp/test
	cd tmp/test ;\
	unzip ../../$< ; \
	latex $(STRIPPED)

clean:
	rm $(NAME).zip

